Multi-criteria Token Fusion with One-step-ahead Attention for Efficient Vision Transformers

Vision Transformer (ViT) has emerged as a prominent backbone for computer vision. For more efficient ViTs, recent works lessen the quadratic cost of the self-attention layer by pruning or fusing the redundant tokens. However, these works faced the speed-accuracy trade-off caused by the loss of information. Here, we argue that token fusion needs to consider diverse relations between tokens to minimize information loss. In this paper, we propose a Multi-criteria Token Fusion (MCTF), that gradually fuses the tokens based on multi-criteria (e.g., similarity, informativeness, and size of fused tokens). Further, we utilize the one-step-ahead attention, which is the improved approach to capture the informativeness of the tokens. By training the model equipped with MCTF using a token reduction consistency, we achieve the best speed-accuracy trade-off in the image classification (ImageNet1K). Experimental results prove that MCTF consistently surpasses the previous reduction methods with and without training. Specifically, DeiT-T and DeiT-S with MCTF reduce FLOPs by about 44% while improving the performance (+0.5%, and +0.3%) over the base model, respectively. We also demonstrate the applicability of MCTF in various Vision Transformers (e.g., T2T-ViT, LV-ViT), achieving at least 31% speedup without performance degradation. Code is available at https://github.com/mlvlab/MCTF.

==> Figures/Figure_sup1.tex <==
 \begin{wrapfigure}{r}{0.45\textwidth}
    \vspace{-25pt}
    \begin{center}
       \includegraphics[trim=0 0 0 0,clip, width=0.45\textwidth]{Figures/loss.png}
      
    \end{center}
    \vspace{-15pt}
    \caption{\textbf{Information loss of MCTF per block.}}
    \label{fig:loss}
 \end{wrapfigure}



% \vspace{}


==> Figures/fig_hist.tex <==
 \begin{figure}[h!]
    \vspace{-10pt}
    \centering
       \includegraphics[trim=0 0 0 0,clip,width=0.9\linewidth]{Figures/hist_size.png}
       \vspace{-10pt}
\caption{\textbf{Histogram of the size of tokens after reduction.}}
\label{fig:hist}
\vspace{-10pt}
 \end{figure}


==> rebuttal/tab_DETR.tex <==
\begin{table}[h!]
\vspace{-10pt}
\small
  \centering 
  \caption{MCTF in object detection. Enc. : encoder, Dec. : Decoder}
\vspace{-10pt}
  \label{tab:DETR}
    \centering
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}{l|cccc}
        Method &  FLOPs (Enc.)& FLOPs (Dec.) & AP \\
        \midrule
        DETR & 9.5 (G) & 1.9 (G) & 42.0\\
        % +EViT & 7.2 (G) & 1.5 (G) & 31.8 \\
        % +ToMe & 7.4 (G) & 1.5 (G) & 41.3 \\
        +MCTF & 7.2 (G) & 1.5 (G) & 41.2 \\
  \end{tabular}
\vspace{-10pt}
\end{table} 

==> rebuttal/tab_abl1.tex <==
\begin{table}[h!]
\vspace{-10pt}
\small
  \centering 
  \caption{Ablations on multi-criteria. $r$ : reduced \# per block}
\vspace{-10pt}
  \label{tab:abl1}
    \centering
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{l|cccc}
        Criteria & $r$=8 & $r$=12 & $r$=16 & $r$=20\\
        \midrule
        Sim. &  79.9 & 79.6 & 79.4 & 77.1 \\
        Sim. + Info. &  \textbf{80.0} & 79.9 & 79.8 & 79.1\\
        Sim. + Info. + Size & \textbf{80.0} & \textbf{80.0} & \textbf{80.1} & \textbf{79.5}\\
  \end{tabular}
\vspace{-10pt}
\end{table} 

==> rebuttal/tab_abl2.tex <==
\begin{table}[h!]
\vspace{-10pt}
\small
  \centering 
  \caption{Ablations on bidirectional bipartite soft matching.}
\vspace{-10pt}
  \label{tab:abl2}
    \centering
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{l|ccccc}
        matching & r=16 & r=17 &  r=18 & r=19 & r=20\\
        \midrule
        One-way. &80.0 & 79.9 & 79.7 & 79.5 & 79.2\\
        Bi. &  \textbf{80.1} & \textbf{80.0} & \textbf{79.9} & \textbf{79.8} & \textbf{79.5}\\
  \end{tabular}
\vspace{-10pt}
\end{table} 

==> rebuttal/tab_lam.tex <==
\begin{table}[h!]
\vspace{-10pt}
\small
  \centering 
  \caption{Sensitivity analyses on $\lambda$ in DeiT-S.}
\vspace{-10pt}
  \label{tab:lam}
    \centering
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{c|cccccccc}
        $\lambda$=0 & $\lambda$=0.1 & $\lambda$=0.5 & $\lambda$=1 & $\lambda$=2 & $\lambda$=3 & $\lambda$=4 & $\lambda$=5 & $\lambda$=10\\
        \midrule
         79.8 & 79.9 & 80.0 & 80.0& 80.0& \textbf{80.1} &80.0&80.0&79.7\\
  \end{tabular}
\vspace{-10pt}
\end{table} 

==> rebuttal/tab_train.tex <==
\begin{table}[t!]
% \vspace{-10pt}
\small
  \centering 
  \caption{Comparison of training time cost.}
\vspace{-10pt}
  \label{tab:train}
    \centering
    \setlength{\tabcolsep}{2pt}
    \resizebox{\linewidth}{!}{\begin{tabular}{l|ccccccc}
         & DeiT-S & AViT & EViT & DyViT & ATS & ToMe & MCTF\\
        \midrule
        Inference FLOPs (G) & 4.6 & 3.6 & 3.0 & 2.9 & 2.9 & 2.7 & \textbf{2.6} \\
        Top-1 accuracy (\%) & 79.8 & 78.6 & 79.5 & 79.3 & 79.7 & 79.4 & \textbf{80.1}\\
        Training time (s) & 256 & 366 & 297 & 554 & 633 & 219 & 595 \\
  \end{tabular}}
\vspace{-20pt}
\end{table}

==> rebuttal_guideline.tex <==
%%%%%%%%% TITLE - PLEASE UPDATE
\title{\LaTeX\ Guidelines for Author Response}  % **** Enter the paper title here

\maketitle
\thispagestyle{empty}
\appendix

%%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW
\section{Introduction}

After receiving paper reviews, authors may optionally submit a rebuttal to address the reviewers' comments, which will be limited to a {\bf one page} PDF file.
Please follow the steps and style guidelines outlined below for submitting your author response.

The author rebuttal is optional and, following similar guidelines to previous conferences, is meant to provide you with an opportunity to rebut factual errors or to supply additional information requested by the reviewers.
It is NOT intended to add new contributions (theorems, algorithms, experiments) that were absent in the original submission and NOT specifically requested by the reviewers.
You may optionally add a figure, graph, or proof to your rebuttal to better illustrate your answer to the reviewers' comments.

Per a passed 2018 PAMI-TC motion, reviewers should refrain from requesting significant additional experiments for the rebuttal or penalize for lack of additional experiments.
Authors should refrain from including new experimental results in the rebuttal, especially when not specifically requested to do so by the reviewers.
Authors may include figures with illustrations or comparison tables of results reported in the submission/supplemental material or in other papers.

Just like the original submission, the rebuttal must maintain anonymity and cannot include external links that reveal the author identity or circumvent the length restriction.
The rebuttal must comply with this template (the use of sections is not required, though it is recommended to structure the rebuttal for ease of reading).

%-------------------------------------------------------------------------

\subsection{Response length}
Author responses must be no longer than 1 page in length including any references and figures.
Overlength responses will simply not be reviewed.
This includes responses where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.

%------------------------------------------------------------------------
\section{Formatting your Response}

{\bf Make sure to update the paper title and paper ID in the appropriate place in the tex file.}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The top margin should begin 1 inch (2.54 cm) from the top edge of the page.
The bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the page.

Please number any displayed equations.
It is important for readers to be able to refer to any particular equation.

Wherever Times is specified, Times Roman may also be used.
Main text should be in 10-point Times, single-spaced.
Section headings should be in 10 or 12 point Times.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Figure and table captions should be 9-point Roman type as in \cref{fig:onecol}.


List and number all bibliographical references in 9-point Times, single-spaced,
at the end of your response.
When referenced in the text, enclose the citation number in square brackets, for example~\cite{Alpher05}.
Where appropriate, include the name(s) of editors of referenced books.

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{0.5in} \rule{0.9\linewidth}{0pt}}
  %\includegraphics[width=0.8\linewidth]{egfigure.eps}
   \caption{Example of caption.  It is set in Roman so that mathematics
   (always set in Roman: $B \sin A = A \sin B$) may be included without an
   ugly clash.}
   \label{fig:onecol}
\end{figure}

To avoid ambiguities, it is best if the numbering for equations, figures, tables, and references in the author response does not overlap with that in the main paper (the reviewer may wonder if you talk about \cref{fig:onecol} in the author response or in the paper).
See \LaTeX\ template for a workaround.

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
Please ensure that any point you wish to make is resolvable in a printed copy of the response.
Resize fonts in figures to match the font in the body text, and choose line widths which render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your response in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the  figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%%%%%%%%% REFERENCES
{
    \small
    \bibliographystyle{ieeenat_fullname}
    \bibliography{main}
}



==> section/method_copy.tex <==
\input{Figures/Figure2}
\section{Method}
\label{sec:3}
% 우리의 목표는 성능 하락없이, 토큰 머징이 합쳐진 모델을 파인튜닝하는것이다.
% We propose a Multi-criteria Token Fusion that progressively combines the token based on multi-criteria to minimize the degradation in the generalization performance of Vision Transformers.
% 3.1 Prelim
% 3.2 MCTF
% 3.3 One-step-ahead attention
% 3.4 Bidirectional bipartite soft matching
% 3.5 Token Reduction Consistency
% Token augmentation consistency에 대한 intuition -> Supplement에 대해 이야기하기, 기존 모델들이 완벽하게 Saturation되지 않음, 그래서 학습을 했을 때, 성능향상 있음 고정한것보다 빠르게 학습 가능
\hjk{
In this section, we review the self-attention and token reduction approaches in~\Cref{sec:3.1}.
Then, we present our multi-criteria token fusion (\Cref{sec:3.2}) that leverages one-step-ahead attention (\Cref{sec:3.3})
and bidirectional bipartite soft matching (\Cref{sec:3.4}). Lastly, we introduce a training strategy with token reduction consistency in~\Cref{sec:3.5}.


\subsection{Preliminaries}
\label{sec:3.1}
In Transformers, tokens $\mathbf{X} \in \mathbb{R}^{N\times C}$ are processed by self-attention defined as 
\begin{align}
\text{SA}(\mathbf{X}) = \text{Softmax}\left(\frac{\mathbf{QK}^\top}{\sqrt{C}} \right) \mathbf{V}, 
\label{eq:SA}
\end{align}
where $\mathbf{Q, K, V} = \mathbf{XW_Q, XW_K,}$ $\mathbf{XW_V}$, and $\mathbf{W_Q, W_K,W_v} \in \mathbb{R}^{C\times C}$ are learnable weight matrices. 
Despite its outstanding expressive power, the self-attention does not scale well with the number of tokens $N$ due to its quadratic time complexity $O(N^2 C + N C^2)$.
To address this problem, 
a line of works~\citep{meng2022adavit,fayyaz2022adaptive,yin2022vit,rao2021dynamicvit, pan2021ia} reduces the number of tokens simply by \textit{pruning} uninformative tokens.
These approaches often cause significant performance degradation due to the loss of information.
Thus, another line of works~\citep{kong2022spvit, liang2022not,marin2023token,bolya2022token,long2023beyond} \textit{fuses} the uninformative or redundant tokens $\hat{\mathbf{X}} \subset \mathbf{X}$ into a new token $\hat{\mathbf{x}} = \delta(\hat{\mathbf{X}})$, where $\mathbf{X}$ is the set of original tokens, and $\delta$ denotes a fusion function, \eg, max-pooling or averaging.
In this work, we also adopt `token fusion' rather than `token pruning' with multiple criteria to minimize the loss of information by token reduction.}
% % While diverse token reduction methods are proposed to lessen the computational cost, considering the multi-criteria for token fusion is still less explored.

% \paragraph{Criteria for token fusion.} 
% \red{To fuse the tokens, the two criteria are mainly considered in previous works, \ie, informativeness, and similarity. 
% As used in~\citep{kong2022spvit, liang2022not, long2023beyond}, informativeness is an effective criterion for token fusion to eliminate the uninformative and meaningless tokens. For these works, the attention map $\mathbf{A} = \text{Softmax}\left(\frac{\mathbf{QK}^\top}{\sqrt{C}} \right)$ of previous self-attention module is tracked and used to measure the informativeness scores $\mathbf{a} \in \mathbb{R}^N$ of the tokens. In parallel, the similarity between the tokens is mainly considered in~\citep{marin2023token, bolya2022token, long2023beyond} to fuse the redundant tokens.}
% While diverse token reduction methods are proposed to lessen the computational cost, considering the multi-criteria for token fusion is still less explored.

% \paragraph{Bipartite soft matching.} 
% To fuse the tokens, redundant tokens should be grouped or matched first. In Token Merging (ToMe)~\citep{bolya2022token}, Bipartite soft matching is introduced to boost the speed of the matching algorithm. For matching, the tokens $\mathbf{x}$ are first split into two groups;
% source tokens and target tokens $\mathbf{X}^\alpha, \mathbf{X}^\beta \in \mathbb{R}^{N^\prime \times C}$, where $N^\prime = N/2$. Then, it calculates the pairwise proximity $\mathbf{W}_{ij} = \mathbf{W}(\mathbf{x}^\alpha_i, \mathbf{x}^\beta_j)$, where $\mathbf{x}^\alpha_i \in \mathbf{X}^\alpha, \mathbf{x}^\beta_j \in \mathbf{X}^\beta$, and $\mathbf{W}$ is the weight measured by similarity metric.
% Given weights, a bipartite graph is generated between $\mathbf{X}^\alpha$ and $\mathbf{X}^\beta$, where the scores of edges $\mathbf{E} \in \mathbb{R}^{N^\prime \times N^\prime}$ defined as
% \begin{align}
%     \mathbf{E}_{ij} &= 
%     \begin{cases}
%     \mathbf{W}_{ij}, & \textnormal{if } j= \arg\max_{j^\prime} \mathbf{W}_{ij^\prime}\\
%     -\infty, & \textnormal{otherwise} 
%     \end{cases}
%     ,
%     \label{eq:edge_tome}
% \end{align}
% which means that each token $\mathbf{x}^\alpha_i$ selects the most similar token in $\mathbf{X}^\beta$. Finally, most similar Top-$r$ edges with high proximity are matched and merged. 
% This matching algorithm introduced the negligible time cost by alleviating the quadratic cost of similarity computation between entire tokens, i.e., $O(N^2 C) \rightarrow O((N^\prime)^2 C)$, where $N^\prime = N/2$, and only using a $\max$ function for matching. 
% Although it boosts the performance and speed over traditional clustering algorithm~\citep{lloyd1982least,kaufman1990partitioning}, there is no chance that redundant tokens in target tokens $\mathbf{X}^\beta$ are fused.


% Also, the model trained with the specific reduction ratio tends to overfit it harming the flexibility.


\subsection{Multi-criteria token fusion}
\label{sec:3.2}
\red{
The goal of MCTF is to generate the set of fused tokens 
\begin{align}
    \hat{\mathbf{X}} = \text{MCTF}(\mathbf{X}; \mathbf{W},r),
    \label{eq:partition}
\end{align}
where $\hat{\mathbf{X}}\in \mathbb{R}^{N-r}$, $\mathbf{W}(\cdot,\cdot)$ is the metric to calculate the weights based on multi-criteria, and $r$ is the reduced number of tokens. 
% In this subsection, we first defines the multi-criteria weights $\mathbf{W}$.
% \begin{align}
%     \hat{\mathbf{X}} = \{\delta({\mathbf{X}_i})\}^{N-r}_i,
%     \label{eq:fusion}
% \end{align}
% where $\hat{\mathbf{X}} \in $ is the $i$-th partition of $\mathbf{X}$, $\mathcal{P}$ is the bidirectional bipartite soft matching (\Cref{sec:3.4}) for partitioning $\mathbf{X}$ into $N-r$ groups, and  $\mathbf{W}(\cdot,\cdot)$ is the metric to calculate the weights based on multi-criteria.
% \red{
% The goal of MCTF is to fuse the tokens based on multi-criteria, which is formulated as
% \begin{align}
%     \{ \mathbf{X}_i \}^{N-r}_i = \text(\mathbf{X}; \mathbf{W},r),
%     \label{eq:partition}
% \end{align}
% \begin{align}
%     \hat{\mathbf{X}} = \{\delta({\mathbf{X}_i})\}^{N-r}_i,
%     \label{eq:fusion}
% \end{align}
% where $\mathbf{X}_i$ is the $i$-th partition of $\mathbf{X}$, $\mathcal{P}$ is the bidirectional bipartite soft matching (\Cref{sec:3.4}) for partitioning $\mathbf{X}$ into $N-r$ groups, and  $\mathbf{W}(\cdot,\cdot)$ is the metric to calculate the weights based on multi-criteria.
In this subsection, we first define the multi-criteria based weights as
\begin{align}
    \mathbf{W}(\mathbf{x}_i, \mathbf{x}_j) = \Pi^M_{k=1}(\mathbf{W}^k(\mathbf{x}_i, \mathbf{x}_j))^{\tau_\mathbf{k}},
\end{align}
where $\mathbf{W}^k(\cdot, \cdot)$ is the weights computed by $k$-th criterion, and $\tau^k$ is the temperature parameters to adjust the influence of each criterion.}
In this work, we consider the following criteria for $\mathbf{W}^k$.
\paragraph{Similarity.}
% Sole criterion, informativeness, sometimes fuses the tokens with fully different semantic information as shown in~\Cref{fig:2.b}. To alleviate this issue, we also consider the similarity between the set of tokens $\mathbf{X}$.
The first criterion is the similarity of the tokens to reduce the redundancies in the set of tokens. Akin to the previous works~\citep{marin2023token, bolya2022token} requiring the proximity of tokens, we calculate the cosine similarity between the set of tokens:
\begin{align}
    \mathbf{W}^\text{sim}(\mathbf{x}_i, \mathbf{x}_j) = \frac{\mathbf{x}_i \cdot \mathbf{x}_j}{\|\mathbf{x}_i\|\|\mathbf{x}_j\|}.
    \label{eq:w_sim}
\end{align}
Grouping the tokens based on similarity is effective in eliminating the redundant tokens, yet it often excessively combines the informative tokens as in~\Cref{fig:2.b}, and the loss of information is inevitable after fusion. So, we opt for the following criterion, informativeness, as the safeguard to encourage fusing the uninformative and meaningless tokens.

\paragraph{Informativeness.}
To quantify the informativeness, we measure the averaged attention scores $\mathbf{a} \in [0,1]^N$ in the self-attention layer, which indicates the impact of each token on others: $\mathbf{a}_j = \frac{1}{N}\sum^N_i \mathbf{A}_{ij}$, where $\mathbf{A}_{ij} = \text{Softmax}\left(\frac{\mathbf{Q}_i\mathbf{K}_j^T}{\sqrt{C}}\right)$. When $\mathbf{a}_i \rightarrow 0$, there's no influence from $\mathbf{x}_i$ to other tokens.
To build the relation with informativeness scores, we formulate the informative weights as follows:
\begin{align}
    \mathbf{W}^\text{info}(\mathbf{x}_i, \mathbf{x}_j) = \frac{1}{\mathbf{a}_i \mathbf{a}_j},
    \label{eq:w_info}
\end{align}
where $\mathbf{a}_i, \mathbf{a}_j$ are the corresponding scores of $\mathbf{x}_i, \mathbf{x}_j$, respectively. When both tokens are uninformative ($\mathbf{a}_i, \mathbf{a}_j \rightarrow 0$), the weight gets higher ($\mathbf{W}^\text{info}(\mathbf{x}_i, \mathbf{x}_j) \rightarrow \infty$), making two tokens prone to be fused. 
In~\Cref{fig:2.c}, with the weights combined with the similarity and informativeness, the tokens in the foreground object are less fused. 

\paragraph{Size.}
The last criterion is the size of the tokens. Although a fused token is designated to be the representative of the constituent tokens, it is difficult to preserve all the information as the number of constituent tokens increases. So, we encourage the small tokens to have a higher chance of being fused. 
To this end, similar to the informativeness scores, we track the number of constituent tokens $\mathbf{s} \in \mathbb{N}^C$ of each token and define the weights as
\begin{align}
    \mathbf{W}^\text{size}(\mathbf{x}_i, \mathbf{x}_j) = \frac{1}{\mathbf{s}_i \mathbf{s}_j}.
    \label{eq:w_size}
\end{align}
In~\Cref{fig:2.d}, based on the multi-criteria combined with both similarity, informativeness, and size, the foreground tokens are less merged, and the size of each token is moderate.




\subsection{One-step-ahead attention for informativeness}
\label{sec:3.3}
\red{
Compared to other straightforward criteria (\eg, similarity, and size), the informativeness is somewhat hard to estimate.
As an approximation for informativeness, existing works~\citep{kong2022spvit,liang2022not,long2023beyond} use the attention scores in previous attention map with the assumption that attentive tokens at the past attention layer are informative for next operations.
To validate this, we here visualize the attention map of consecutive layers in~\Cref{fig:att_diff}.
Contrary to the assumption, some of the attentive tokens in the previous layer are inattentive in the next layer (and Vice Versa).}
% Namely, if we rely on the previous attention map $\mathbf{A}^{l-1}$, it may fuse the attentive tokens for the subsequent attention layer. 
% Further, we measure the difference between attention maps of consecutive layers ($\|\mathbf{A}^{l-1} - \mathbf{A}^{l}\|$) across the layer and provide it in ??. 
\red{Based on this observation, we demonstrate that if we rely on the previous attention map, it is prone to fuse the attentive tokens in the subsequent self-attention layer. Thus, we opt for the \textbf{one-step-ahead attention}, which is the attention map in the next layer.
% , to estimate the informativeness scores $\mathbf{a}$ of \Cref{eq:w_info} for token fusion.
For one-step-ahead attention, we simply extract the attention map in the following self-attention layer: $\mathbf{\tilde{A}} = \text{softmax}(\frac{\mathbf{Q} \mathbf{K}}{\sqrt{C}})$. Then, the informativeness scores $\mathbf{a}$ of \Cref{eq:w_info} is calculated with $\mathbf{\tilde{A}}\in \mathbb{R}^{N \times N}$.
Although one-step-ahead attention enables to explicitly understand the informativeness for the following operation, one more issue still remains unresolved.
The original attention map $\hat{\mathbf{A}} \in \mathbb{R}^{(N-r) \times (N-r)} $ is also required with the fused tokens $\hat{\mathbf{X}} \in \mathbb{R}^{(N-r) \times C}$ in the self-attention layer.
In other words, the computation of one-step-ahead attention brings additional quadratic costs of the similarity calculation.
To mitigate the complexity, we approximate $\hat{\mathbf{A}}$ with one-step-ahead attention $\tilde{\mathbf{A}}$ by fusing the attention scores itself.
For instance, when the partitioned tokens $\mathbf{X}_i$ are fused as in~\Cref{eq:fusion}, their corresponding one-step-ahead attention scores $\mathbf{A}_i$ is also fused as
\begin{align}
    \hat{\mathbf{A}} = \{\delta(\tilde{\mathbf{A}}_i)\}^{N-r}_i.
    \label{eq:approx_att}
\end{align}
}
After fusion of the one-step-ahead attention in both query and key direction, we can approximate $\hat{\mathbf{A}}$ without extra similarity computation. 
When fusing the key scores, we use the sum for $\delta$ to maintain the sum of attention scores as 1. 

\input{Figures/Figure3}


\input{Figures/Figure4}
\subsection{Multi-criteria Token Fusion}
\label{sec:3.4}
Given the multi-criteria based weights $\mathbf{W}$, MCTF conduct \textbf{Bidirectional bipartite soft matching} for grouping and fusing the tokens.
% Given the set of the tokens $\mathbf{X}$ and multi-criteria-based weights $\mathbf{W^t}$, the next step is to group the tokens for fusion. 
Bipartite soft matching is introduced in ToMe~\citep{bolya2022token} with the negligible cost by alleviating the quadratic cost of similarity computation between tokens, \ie, $O(N^2 C) \rightarrow O((N^\prime)^2 C)$, where $N^\prime = \lfloor \frac{N}{2} \rfloor$. 
In this matching algorithm, the set of tokens $\mathbf{X}$ is first split into the source and target $\mathbf{X}^\alpha, \mathbf{X}^\beta \in \mathbb{R}^{N^\prime \times C}$ as in Step 1 of~\Cref{fig:bi}.
Then, the objective of this matching is to find the edge matrix $\mathbf{E} \in \{0,1\}^{N' \times N'}$ between $\mathbf{X}^\alpha, \mathbf{X}^\beta$, which is formalized as
\begin{align}
    &\argmax_{\mathbf{E}} \sum \mathbf{w}^\prime_{ij} \mathbf{e}_{ij}\\
    &\text{subject to} \sum \mathbf{e}_{ij} = r, \nonumber \\
    &\quad\quad\quad\quad\;\;\mathbf{w}^\prime_{ij} = \begin{cases}
    \mathbf{w}_{ij} & \text{if } j \neq \argmax_{j^\prime} \mathbf{w}_{ij^\prime}\\
    0 & \text{otherwise}
    \end{cases}, \nonumber 
\end{align}
where $\mathbf{e}_{ij}$ indicates the presence of the edge between $i,j$-th token of $\mathbf{X}^\alpha, \mathbf{X}^\beta$, and $\mathbf{w}_{ij} = \mathbf{W}(\mathbf{x}^\alpha_i, \mathbf{x}^\beta_j)$.
% In this matching algorithm, the set of tokens $\mathbf{X}$ is first split into the source and target $\mathbf{X}^\alpha, \mathbf{X}^\beta$ as in Step 1 of~\Cref{fig:bi}.
% Then, we calculate the pairwise weights and build the bipartite graph $\mathbf{E}^\alpha$ defined as%~\Cref{eq:edge_tome}
% \begin{align}
%     \mathbf{E}_{ij} &= 
%     \begin{cases}
%     \mathbf{W}^t_{ij}, & \textnormal{if } j= \arg\max_{j^\prime} \mathbf{W}^t_{ij^\prime}\\
%     -\infty, & \textnormal{otherwise} 
%     \end{cases}
%     ,
%     \label{eq:edge_tome}
% \end{align}
% where $\mathbf{W}^t_{ij} = \mathbf{W}^t(\mathbf{x}^\alpha_i, \mathbf{x}^\beta_j)$, and $\mathbf{x}^\alpha_i, \mathbf{x}^\beta_j$ are the $i ,j$-th tokens of $\mathbf{X}^\alpha, \mathbf{X}^\beta$, respectively.
Namely, each token $\mathbf{x}^\alpha_i$ selects one of the tokens having the highest weights in $\mathbf{X}^\beta$, and the top-$r$ matchings are selected. Then, based on $\mathbf{E}$, we group the tokens as
\begin{align}
&\mathbf{X}^{\alpha \rightarrow \beta}_i = \{\mathbf{x}^\alpha_j \in \mathbf{X}^\alpha \; | \; \mathbf{e}_{ij} =1\} \cup \{\mathbf{x}^\beta_i\},
\end{align}
where $\mathbf{X}^{\alpha\rightarrow\beta}_i$ indicates the set of tokens matched with $\mathbf{x}^\beta_i$.
Finally, the partitioning results with $\mathbf{X}^{\alpha \rightarrow \beta}_i$ is defined as
\begin{align} 
&\mathcal{P}(\mathbf{X}; \mathbf{W},r)= \{\{\tilde{\mathbf{x}}^\alpha_i\}\}^{N^\prime-r}_i \cup \{\mathbf{X}^{\alpha \rightarrow \beta}_i\}^{N^\prime}_i,
% &\mathbf{X}^{\alpha \rightarrow \beta}_i = \{\mathbf{x}^\alpha_j \in \mathbf{X}^\alpha \; | \; \mathbf{e}_{ij} =1\} \cup \{\mathbf{x}^\beta_i\},
\end{align}
where $\tilde{\mathbf{x}}^\alpha_i$ is the $i$-th token of $\tilde{\mathbf{X}}^\alpha =  \mathbf{X}^\alpha - {\bigcup}^{N^\prime}_i \mathbf{X}^{\alpha \rightarrow \beta}_i$.
Now, through~\Cref{eq:fusion} with pooling operation $\delta(\mathbf{X}) = \delta(\{\mathbf{x}_i\}_i)= \sum_i \frac{\mathbf{a}_i\mathbf{s}_i\mathbf{x}_i}{\sum_{i^\prime} \mathbf{a}_{i^\prime}\mathbf{s}_{i^\prime}}$ considering the attention scores $\mathbf{a}$ and the size $s$ of the tokens, we obtain fused set of tokens.
However, as shown in Step2 of~\Cref{fig:bi}, there is no chance that tokens in target tokens $\mathbf{X}^\beta$ are fused in this one-way bipartite matching.
% attentive sum defined as $\delta(\{\mathbf{x}_i\}_i) = \sum_i \frac{\mathbf{a}_i \mathbf{x}_i}{\sum_j \mathbf{a}_j}$.
To handle this issue, with updated two sets of the tokens $\tilde{\mathbf{X}}^\alpha \in \mathbb{R}^{(N^\prime - r) \times C}, \tilde{\mathbf{X}}^\beta \in \mathbb{R}^{N^\prime \times C}$, same process is repeated in Step 3, 4 of the figure after swapping the source and target resulting in fused tokens $\hat{\mathbf{X}} = \hat{\mathbf{X}}^\alpha \cup \hat{\mathbf{X}}^\beta $, where
\begin{align}
    &\hat{\mathbf{X}}^\alpha = \{\delta(\tilde{\mathbf{X}}^{\beta \rightarrow \alpha}_i)\}^{N^\prime-r}_i, \label{eq:x_hat_a}\\
    &\hat{\mathbf{X}}^\beta  = \mathbf{X}^\beta - {\bigcup}_i \tilde{\mathbf{X}}^{\beta \rightarrow \alpha}_i
    .
    \label{eq:x_hat_b}
\end{align}
Note that calculating the pairwise weights with updated two sets of tokens $\mathbf{W}^\mathbf{t} (\tilde{\mathbf{x}}^\beta_i, \tilde{\mathbf{x}}^\alpha_j)$  introduces the additional computational costs of $O(N^\prime (N^\prime - r) C)$. To avoid this overhead, we approximate the weights by considering $\tilde{\mathbf{x}}^\beta_i \simeq  \mathbf{x}^\beta_j$. Then, since $\tilde{\mathbf{X}}^\alpha$ is the subset of $\mathbf{X}^\alpha$, we can reuse the pre-calculated weights. As a result, we could reduce the tokens with MCTF considering bidirectional relations between two subsets with negligible extra costs compared to one-way.


% Whereas, during the fusion with query direction, we adopt \Cref{eq:fusion} for a better approximation of original $\hat{A}^l$


% During the matching, if the tokens $\{\mathbf{x}^l_i\}_i \in \mathbf{X}^l$ is fused, then we fuse its attention score $\{\mathbf{A}^l_i\}_i$, too. For instance, the one-step-ahead attention is split and grouped corresponding to the token matching.
% Since $\mathbf{A}^l_i \in \mathbb{R}^N$ indicates the attention scores with respect to query $\mathbf{x}^l_i \in \mathbf{X}^l$, we simply fuse the attention scores when the tokens fused.
% $\hat{\mathbf{A}}^l_{ij}$ is the attention score with key $\hat{\mathbf{x}}_i$ and query $\hat{\mathbf{x}}_j$ and $\hat{\mathbf{X}}$ is the results of MCTF.


% since the attention map required for updating the , 
% After the MCTF operation, the fused tokens $\hat{\mathbf{X}}^l$ are updated with the self-attention layer. 
% Note that, 

% In MCTF, we adopt pre-attention for an informativeness score. Given $\mathbf{X}^{l}$, the pre-attention $\mathbf{A}^{l+1}$ is first calculated. Then, MCTF is conducted to generated the tokens $\hat{\mathbf{X}}^$ 

% In previous works, post-attention, which is already used in previous self-attention, is a mainly used criterion to measure the informativeness of each token. 


% In previous works, post-attention, which is the attention map of the previous self-attention operation, is the prevalent choice to evaluate the informativeness of each token. In these works, the inattentive tokens are fused based on post-attention scores with the belief that the attentive tokens are also informative in the next layer. 
% However, these works overlook the fact that the attention maps in consecutive layers vary significantly. In ???, we visualize the attention map in consecutive layers. 
% As shown in the figure, some of the attentive tokens in -th layer are inattentive in the next layer (and Vice Versa). 
% In other words, with post-attention, informative tokens at the next layer can be fused resulting in the loss of information. Further, considering that post-attention is already used in previous self-attention, 


% the pre-attention, which is a pre-calculated attention map for the next self-attention, should be considered. 
%In the token fusions~\citep{kong2022spvit, liang2022not,long2023beyond} designed with informativeness, an attention map in the previous self-attention layer is the prevalent choice to evaluate the informativeness of each token. In these works, the inattentive tokens are fused based on the attention map of the previous self-attention operation with the belief that the attentive tokens are also informative in the next layer.
% However, this post-attention, which is already used in previous self-attention, is 
% the inattentive tokens having lower attention scores are fused with the belief that the attentive tokens are more informative. 
%Further, considering that pre-attention is already 
%In other words, previous works are prone to merge the 
%Note that, if we fuse the tokens between these two layers, 
%Further, considering that if we fuse the tokens afte
%For instance, in ???, we visualize the attention maps in the ??-th and ??-th layers of the ViTs. Note that, if we fuse the tokens between these two layers, 
% using the informativness for criterion 
% 하지만 위와 같은 연구들은 심지어 연속되는 layer에서 조차 attention map이 크게 다를 수 있다는 사실을 간과하고 있다.


% Although MCTF boosts the performance, it does not guarantees that multi-cirteria actually prevents the loss of information. Here, we  

% Unlike previous works only considering the one criterion, our MCTF opt the multi-criterion for matching relative tokens. Specifically, we incorporate three criteria: (1) similarity of the tokens, (2) informativeness, and (3) size of the tokens. 

% \input{Figures/Figure4}

\input{Figures/Figure5}
\subsection{Token reduction consistency}
\label{sec:3.5}
In this work, we train vision Transformer $f_\theta(\cdot;r)$ with MCTF considering two aspects of token reduction methods. First, as the number of reduced tokens per layer, $r$, increases, the representation of the sample is also largely changed. In other words, by adjusting $r$, we can control the difficulty of the sample, which can be seen as token-level augmentation. Second, at the same time, the global representations of the input $x$ should be consistent regardless of the reduction ratio, since they represent the same sample. Herein, we propose the training objective combined with the token augmentation consistency via random reduction:
\begin{align}
    \mathcal{L} = \mathcal{L}_\text{CE}(f_\theta(x,r), y) &+ \mathcal{L}_\text{CE}(f_\theta(x,r^\prime), y) \nonumber \\
    &+  \lambda\mathcal{L}_\text{MSE}(\mathbf{x}^\text{cls}_r, \mathbf{x}^\text{cls}_{r^\prime})
    ,
    \label{eq:con}
\end{align}
where $(x,y)$ is the paired data, $r, r^\prime$ is the fixed and dynamic reduction ratio, $\lambda$ is the coefficient for consistency loss, and $\mathbf{x}^\text{cls}_r, \mathbf{x}^\text{cls}_{r^\prime}$ is the class token in the last layer of $f_\theta(x;r), f_\theta(x;r^\prime)$ .
In this objective, we first calculate the cross-entropy loss $\mathcal{L}_\text{CE}(f_\theta(x,r), y)$ with fixed $r$, which is the target reduction ratio that will be used in the evaluation. 
At the same time, to generate the augmented representation of the input $x$, we forward the input with dynamically varying $r^\prime \in [0,r]$, and calculate the loss $\mathcal{L}_\text{CE}(f_\theta(x,r^\prime), y)$, too. Then, introducing the consistency loss $\mathcal{L}_\text{MSE}(\mathbf{x}^\text{cls}_r, \mathbf{x}^\text{cls}_{r^\prime})$ on the class tokens, we hope the model to retain the consistent representation across the diverse number of reduced tokens bypassing the loss of information. A more detailed analysis of token reduction consistency, including intuition for design choices, is presented in supplement with experiments.
%Similar to UDA~\cite{xie2020unsupervised}, the consistency loss is calculated only with the sample that the model is confident about.





% Given the Transformer model $f_\theta$, we build the model $f_\theta(\cdot;r)$ by combining MCTF at the last of each block, where $r$ indicates the number of tokens reduced per layer. 

% Data augmentation is the key to improving the generalization ability of the model. 
%token-level augementation


%Here, we introduce the new training objective with token


% Similar to previous works, we observed the performance degradation with $f^\prime$ due to the reduced complexity. To mitigate the problem, we here propose the new training objective for token reduction methods with self-distillation. 
% Knowledge distillation (\textbf{KD}) is the concept to transfer the knowledge of a large teacher model to another small student model. Given the student model $f_S$ and $f_T$, the student learns from the soft label of the teacher model's prediction with the distillation loss:
% \begin{align}
%     \mathcal{L}_\text{KD}(f_S,f_T,x;\tau) = \mathcal{L}_\text{CE}(f_S(x;\theta_S,\tau), f_T(x;\theta_T,\tau))
%     ,
%     \label{eq:KD}
% \end{align}
% where $L_\text{CE}$ is the cross-entropy loss and $\tau$ is the temperature to adjust the smoothness of the label. In our settings, we assume the base model $f$ as the teacher model for the student model $f^\prime$ instead of introducing additional teacher networks. The two models share the same architectures and parameters ($\theta_S$ = $\theta_T = \theta$) except for MCTF operation, which can be seen as self-knowledge distillation (\textbf{SD}). 
% Then, integrating with the classification loss $\ell_f = L_\text{CE}(f(x; \theta),y)$ with hard label $y$, our objective loss can be written as:
% \begin{align}
%     \mathcal{L} = \ell_f+ \ell_{f^\prime} + 
%     \alpha \ell_{SD}
%     % \mathcal{L}_\text{KD}(f,f_\text{MCTF};x,\tau)
%     \label{eq:total_loss}
%     ,
% \end{align}
% where $\ell_\text{SD} = \mathcal{L}_\text{KD}(f,f^\prime,x;\tau)$. Interestingly, we empirically observed that instead of the soft label, predicting the teacher's class token of the last block brings more improvement based on 
% \begin{align}
% \ell_\text{SD} = \mathcal{L}_\text{MSE}(\mathbf{x}_\text{cls}, \mathbf{x}_\text{cls}^\prime),
% \label{eq:SD}
% \end{align}
% where $\mathbf{x}_\text{cls}, \mathbf{x}_\text{cls}^\prime$ is the class token of $f, f^\prime$ (see \Cref{fig:SD}). We demonstrate that this simple change explicitly helps prevent information loss in the class token. See~\Cref{sec:4.2} for comparisons of $\ell_{SD}$ choices. The pseudo-code for training with self-distillation is provided in \Cref{alg:SD}.

% Note that DynamicViT~\citep{rao2021dynamicvit} uses a similar distillation loss on the remained tokens and predicted logits between the student and pre-trained teacher model ($\theta_S \neq \theta_T)$. Whereas, in our self-distillation, since the teacher model shares the same parameters and architectures, we train the model without a pre-trained one. As a result, our proposed loss is more flexible with diverse Transformers. 


==> tables/table_abl2.tex <==
\begin{table*}[t!]
  \centering 
  % \begin{subtable}[h]{0.45\textwidth}
  \begin{minipage}{.32\linewidth}
  \caption{\textbf{Comparison of pooling function $\delta$}}
  \label{tab:abl2}
  \begin{tabular}{lcc}
        \toprule
        \multicolumn{1}{c}{$\delta$} & im/s & Acc\\
        \midrule
        avg          & 2067 &     79.6      \\
        max          & 2081 &     79.5      \\
        w.avg        & 2047 &     79.7      \\
        att.sum      & 2021 & \textbf{79.9} \\
        \bottomrule
  \end{tabular}
  \end{minipage} 
  \hfill
  \begin{minipage}{.32\linewidth}
  \caption{\textbf{Comparison of matching function}}
  \label{tab:abl3}
  \begin{tabular}{lcc}
        \toprule
        \multicolumn{1}{c}{matching} & im/s & Acc\\
        \midrule
        \multirow{2}{*}{one-way}  & \multirow{2}{*}{2042}  & \multirow{2}{*}{79.8} \\
        \\
        \multirow{2}{*}{bi.}      & \multirow{2}{*}{2021} & \multirow{2}{*}{\textbf{79.9}} \\
        \\
        \bottomrule
  \end{tabular}
  \end{minipage}
  \hfill
  \begin{minipage}{.32\linewidth}
  \caption{\textbf{Comparison of self-knowledge distillation loss}}
  \label{tab:abl4}
  \begin{tabular}{lcc}
        \toprule
        \multicolumn{1}{c}{$\ell_\text{SD}$} & im/s & Acc\\
        \midrule
        pred        & 2021 & 79.8 \\
        entire cls  & 2021 & 79.6 \\
        last cls    & 2021 & \textbf{79.9} \\
        \\
        \bottomrule
  \end{tabular}
  \end{minipage}

% \vspace{-10pt}
\end{table*} 
